Clusterization in D-optimal designs: the case against linearization

Estimation of parameters in physical processes often demands costly measurements, prompting the pursuit of an optimal measurement strategy. Finding such strategy is termed the problem of optimal experimental design, abbreviated as optimal design. Remarkably, optimal designs can yield tightly clustered measurement locations, leading researchers to fundamentally revise the design problem just to circumvent this issue. Some authors introduce error correlation among error terms that are initially independent, while others restrict measurement locations to a finite set of locations. While both approaches may prevent clusterization, they also fundamentally alter the optimal design problem. In this study, we consider Bayesian D-optimal designs, i.e.~designs that maximize the expected Kullback-Leibler divergence between posterior and prior. We propose an analytically tractable model for D-optimal designs over Hilbert spaces. In this framework, we make several key contributions: (a) We establish that measurement clusterization is a generic trait of D-optimal designs for linear inverse problems with independent Gaussian measurement errors and a Gaussian prior. (b) We prove that introducing correlations among measurement error terms mitigates clusterization. (c) We characterize D-optimal designs as reducing uncertainty across a subset of prior covariance eigenvectors. (d) We leverage this characterization to argue that measurement clusterization arises as a consequence of the pigeonhole principle: when more measurements are taken than there are locations where the select eigenvectors are large and others are small -- clusterization occurs. Finally, we use our analysis to argue against the use of Gaussian priors with linearized physical models when seeking a D-optimal design.

==> how.tex <==
%\section{Clusterization poses no obstruction to D-optimality}\label{section:clusterization}
\section{Substituting an optimal clustered design with an equally optimal non-clustered design}\label{section:how}
%
The necessary conditions for D-optimality of Theorem \ref{thm:char}
leave some freedom in choosing $\obs$, which might allow us to avoid a
clustered design. As an example, consider an inverse problem for which
the first two eigenvalues of the pushforward prior $\fwd \prcov\fwd^*$
are $\lambda_1 = 10, \lambda_2 = 5$, with eigenvectors
$\{\ev_i\}_{i=1}^\infty$ and $\sigma^2=1$. Consider the following
$\obs, \pobs$ (see also Fig.~\ref{fig:clusterization}):
\begin{equation}\label{eq:two_designs}
  \obs =
  \begin{pmatrix}
    \sqrt{\frac{11}{40}}\ev_1 - \sqrt{\frac{29}{40}}\ev_2 \\
    \sqrt{\frac{11}{40}}\ev_1 + \sqrt{\frac{29}{40}}\ev_2 \\
    \ev_1 \\
    \ev_2 \\
    \ev_1 \\    
  \end{pmatrix},
  \pobs =
  \begin{pmatrix}
    \sqrt{\frac{3}{8}}\ev_1 - \sqrt{\frac{5}{8}}\ev_2 \\
    \sqrt{\frac{3}{8}}\ev_1 + \sqrt{\frac{5}{8}}\ev_2 \\
    \sqrt{\frac{2}{5}}\ev_1 - \sqrt{\frac{3}{5}}\ev_2 \\
    \sqrt{\frac{2}{5}}\ev_1 + \sqrt{\frac{3}{5}}\ev_2 \\
    \ev_1 \\    
  \end{pmatrix}
\end{equation}
\noindent It is easy to verify that $\obs^*\obs = \pobs^*\pobs$
and that both $\obs$ and $\pobs$ are D-optimal. However, $\obs$
is a clustered design ($\meas_3 = \meas_5 = \ev_1$), while $\pobs$ is
not.

We may now answer \textbf{Question \ref{q:replace}}: We showed that it
is possible to substitute a D-optimal clustered design (e.g. $\obs$)
for a D-optimal non-clustered design (e.g. $\pobs$). Presenting a
general algorithm for replacing a clustered D-optimal design with a
non-clustered D-optimal design is out of the scope of the current
study. We can, however, provide some intuition, utilizing $\obs,
\pobs$ as a test case. Let $\obs_{12}$ the design composed of the
first and second rows of $\obs$ (with a similar definition for
$\pobs_{12}$), and note that, up to permutations and sign changes,
$\obs_{12}$ uniquely determines $\obs$ as a clustered design. We find
$\pobs_{12}$ by requiring that (a) measurements in $\pobs_{12}$ have
unit norm, (b) $\pobs_{12}^* \pobs_{12}$ has the same eigenvectors as
$\obs^*\obs$, (c) $\pobs^*\pobs \approx \obs^*\obs$, and (d)
$\pobs^*\pobs \neq \obs^*\obs$. We then consider a ``new'' inverse
problem, for which the pushforward prior covariance is the covariance
of the posterior $\mu_{\textup{post}}^{\data, \pobs_{12}}$, namely

$$
\left(\left(\fwd \prcov\fwd^*\right)^{-1} + \sigma^{-2}
\pobs_{12}^*\pobs_{12}\right)^{-1}.
$$
%
Finally, we complete $\pobs$ to a D-optimal design with $m=5$
measurements via the construction outlined in Lemma
\ref{lemma:free}.

Interestingly, part (c) in the process detailed above implies that
there are actually infinitely many non-clustered D-optimal designs. It
is not at all clear why the numerical implementation of Lemma
\ref{lemma:free} results in a clustered design. An answer to this
question may further help shed light on the measurement clusterization
phenomenon.


\pgfplotstableread{
  Label    prior  $o_1o_2$  $o_3$   $o_4$   $o_5$    topper
  1         0.1      0.55       1       0       1      0.001
  2         0.2      1.45       0       1       0      0.001
  3         3.5      0          0       0       0      0.001
}\clusterization


\pgfplotstableread{
  Label    prior  $o_1o_2$  $o_3o_4$   $o_5$     topper
  1         0.1    0.75     0.8        1         0.001
  2         0.2    1.25     1.2        0         0.001
  3         3.5    0        0          0         0.001
}\noclusterization

\begin{figure}
  \begin{tikzpicture}[scale=0.85]
    \begin{axis}[
        ybar stacked,
        ymin=0,
        ymax=4,
        xtick=data,
        legend style={cells={anchor=east}, legend pos=north west, legend columns=-1},
        reverse legend=false, % set to false to get correct display, but I'd like to have this true
        xticklabels from table={\clusterization}{Label},
        xticklabel style={text width=2cm,align=center},
        legend plot pos=right,
        ylabel=precision --- prior and posterior,
        xlabel=eigenvector $i$,
      ]
    
      
      \addplot [fill=green!80]  table [y=prior, meta=Label, x expr=\coordindex] {\clusterization};
      \addplot [fill=blue!60]   table [y=$o_1o_2$, meta=Label, x expr=\coordindex] {\clusterization};
      \addplot [fill=red!60]    table [y=$o_3$, meta=Label, x expr=\coordindex] {\clusterization};
      \addplot [fill=black!60]  table [y=$o_4$, meta=Label, x expr=\coordindex] {\clusterization};
      \addplot [fill=orange!60] table [y=$o_5$, meta=Label, x expr=\coordindex] {\clusterization};
      %% \addplot [fill=cyan!60]   table [y=$o_6$, meta=Label, x expr=\coordindex] {\clusterization};
      %% \addplot [fill=purple!60] table [y=$o_7$, meta=Label, x expr=\coordindex] {\clusterization};

      
      \addlegendentry{prior}
      \addlegendentry{$o_1o_2$}
      \addlegendentry{$o_3$}
      \addlegendentry{$o_4$}
      \addlegendentry{$o_5$}
      %% \addlegendentry{$o_6$}
      %% \addlegendentry{$o_7$}   
    \end{axis}
  \end{tikzpicture}
  \qquad
  \begin{tikzpicture}[scale=0.85]
    \begin{axis}[
        ybar stacked,
        ymin=0,
        ymax=4,
        xtick=data,
        legend style={cells={anchor=east}, legend pos=north west, legend columns=-1},
        reverse legend=false, % set to false to get correct display, but I'd like to have this true
        xticklabels from table={\noclusterization}{Label},
        xticklabel style={text width=2cm,align=center},
        legend plot pos=right,
        ylabel=precision --- prior and posterior,
        xlabel=eigenvector $i$,
      ]
    
      
      \addplot [fill=green!80]  table [y=prior, meta=Label, x expr=\coordindex] {\noclusterization};
      \addplot [fill=blue!60]   table [y=$o_1o_2$, meta=Label, x expr=\coordindex] {\noclusterization};
      \addplot [fill=red!60]    table [y=$o_3o_4$, meta=Label, x expr=\coordindex] {\noclusterization};
      \addplot [fill=black!60]  table [y=$o_5$, meta=Label, x expr=\coordindex] {\noclusterization};
      %% \addplot [fill=orange!60] table [y=$o_4$, meta=Label, x expr=\coordindex] {\noclusterization};
      %% \addplot [fill=cyan!60]   table [y=$o_5$, meta=Label, x expr=\coordindex] {\noclusterization};
      %% \addplot [fill=purple!60] table [y=$o_6$, meta=Label, x expr=\coordindex] {\noclusterization};

      
      \addlegendentry{prior}
      \addlegendentry{$o_1o_2$}
      \addlegendentry{$o_3o_4$}
      \addlegendentry{$o_5$}
      %% \addlegendentry{$o_4$}
      %% \addlegendentry{$o_5$}
      %% \addlegendentry{$o_6$}   
    \end{axis}
  \end{tikzpicture}
  \caption{Clusterization (left, $\obs$ in \eqref{eq:two_designs})
    and non-clusterization (right, $\pobs$ in \eqref{eq:two_designs})
    in D-optimal designs. Posterior precision per eigenvector is
    plotted for $\obs$ and $\pobs$ from \eqref{eq:two
______designs}. Both designs are identical for all practical matters
    --- their posteriors are equal. In the left panel, a D-optimal
    design with clusterization is illustrated: $\meas_3 = \meas_5$. In
    the right panel, a D-optimal design without clusterization is
    illustrated. The contribution to the posterior precision due to
    $\meas_1$ and $\meas_2$ is denoted $\meas_1\meas_2$. These
    contributions are plotted together because neither $\meas_1$ nor
    $\meas_2$ are not in the direction of any eigenvector. Similarly
    for $\meas_3\meas_4$.}
  \label{fig:clusterization}
\end{figure}


==> why.tex <==
\subsection{Answer to Question \ref{q:why}}\label{subsec:why}
Building on Theorem \ref{thm:char}, we can now give a compelling
explanation to the measurement clusterization we observed for the
inverse problem of the heat equation, see Section
\ref{subsub:clusterization1} below. We also suggest a generic
explanation for clusterization, see Section \ref{subsub:clusterization2}.

\subsubsection{Clusterization in the heat equation}
Consider $\fwd$ and $\prcov$ from \emph{the inverse problem of the
heat equation}. As before, we denote the eigenvalues of
$\fwd\prcov\fwd^*$ by $\lambda_j$. We input these eigenvalues into our
\emph{generic} model, and find a D-optimal design $\opt$ for our
generic model using Theorem \ref{thm:char}. In our generic model, the
measurements we take are best utilized in reducing uncertainty for the
first $k$ eigenvectors. So, a D-optimal design arising from our
\emph{generic model} completely avoids measuring eigenvectors $k+1$
and above.

Of course, in a real life problem --- such as the inverse problem of
the 1D heat equation --- it is likely impossible to find measurement
locations for which all eigenvectors $k+1$ and above are
zero. However, if the eigenvalues of $\fwd\prcov\fwd^*$ decay quickly
(recall the square-exponential decay for eigenvalues of the 1D heat
equation in eq.\eqref{eq:decay}), a D-optimal design will try to
balance measuring a small number (i.e.~$k$) of the leading
eigenvectors.

The abovementioned balance is explored in
Fig.~\ref{fig:eigenvectors}. We allow $m=4$ measurements in $\Omega =
[0,1]$ and observe that D-optimal measurement locations are clustered
at $x_1 = 0.31$ and $x_2 = 0.69$. Upon close inspection of the scaled
eigenvectors of $\fwd \prcov \fwd^*$, we first observe that
eigenvectors $3$ and above have negligible prior amplitude. Since we
only have $m=4$ measurements at our disposal, we interpret these
results, following Theorem \ref{thm:char}, as implying we should only
care about measuring the first and second eigenvectors. Then, we note
the D-optimal $x_1,x_2$ present a compromise between the amplitude of
the first and second eigenvectors. For example, a measurement at
$x=0.5$ would have ignored the second eigenvector altogether, since
the second eigenvector is zero at $x=0.5$.

Now we can understand measurement clusterization for the inverse
problem of the heat equation. A D-optimal design attempts to measure
the first $k$ eigenvectors of $\fwd \prcov \fwd^*$. But there may be
(spatial) limitations on where these $k$ eigenvectors have large
amplitude. For the inverse problem of the heat equation there are two
spatial locations that present a good compromise between the
amplitudes of the first and second eigenvectors, namely $x_1$ and
$x_2$ --- see Fig.~\ref{fig:eigenvectors}. We have $m=4$ measurements
at our disposal but only two spatial locations that are a good
compromise between the first and second scaled eigenvectors. Thus,
clusterization arises as a consequence of the pigeonhole principle.

\begin{figure}\label{fig:eigenvectors}
    \centering
    \includegraphics[width=\textwidth]{figs/eigenvectors_dst_scaled.png}
    \caption{D-optimal measurement locations ($m=4$ measurements) and
      weighted eigenvectors for finding the initial condition of the
      1D heat equation. Measurement locations and weighted
      eigenvectors are plotted over the computational domain $\Omega =
      [0, 1]$ (x-axis). Measurement clusterization occurs
      approximately at $0.31$ and $0.69$. These two locations are a
      compromise between the magnitudes of the first and second
      eigenvectors, which are the eigenvectors that a D-optimal design
      aims to measure. Allocating $m=4$ measurements into two
      locations results in clusterization, according to the pigeonhole
      principle.}
  \label{fig:why}
\end{figure}

